Free boundary regularity for tumor growth with nutrients and diffusion

In this paper, we study a tumor growth model where the growth is driven by nutrient availability and the tumor expands according to Darcy's law with a mechanical pressure resulting from the incompressibility of the cells. Our focus is on the free boundary regularity of the tumor patch that holds beyond topological changes. A crucial element in our analysis is establishing the regularity of the hitting time T, which records the first time the tumor patch reaches a given point. We achieve this by introducing a novel Hamilton-Jacobi-Bellman (HJB) interpretation of the pressure, which is of independent interest. The HJB structure is obtained by viewing the model as a limit of the Porous Media Equation (PME) and building upon a new variant of the AB estimate. Using the HJB structure, we establish a new Hopf-Lax type formula for the pressure variable. Combined with barrier arguments, the formula allows us to show that T is C^{\alpha}, where \alpha depends only on the dimension, which translates into a mild nondegeneracy of the tumor patch evolution. Building on this and obstacle problem theory, we show that the tumor patch boundary is regular in spacetime except on a set of Hausdorff dimension at most $d-\alpha$. On the set of regular points, we further show that the tumor patch is locally $C^{1,\alpha}$ in space-time. This conclusively establishes that instabilities in the boundary evolution do not amplify arbitrarily high frequencies.

==> old_arguments.tex <==

\textcolor{blue}{In the following Lemma, we give $L^m_tL^{\infty}_x$ bounds on the time derivative of the nutrient variable.  Note that $L^m_tL^{\infty}_x$ cannot be achieved by generic regularity theory for the heat equation with an $L^{\infty}$ source term, which gets stuck at BMO for the usual reasons one sees in elliptic and parabolic regularity theory.  We push for the stronger $L^m_tL^{\infty}_x$ bound so that we can eventually control $u_+$ in a space with super-exponential growth --- a bound that would not be possible if we only had BMO control on $\partial_t n$.  To obtain this stronger bound, we need to exploit the structure of the source term in the nutrient equation and use the fact that $p$ is Holder continuous in space for $d<4$. }
\begin{lemma}\label{lem:dt_n_estimate}
If $d<4$ and $n^0\in W^{1,\infty}(\RR^d)$, then for any $T>0$ and $m\in [1,\infty)$,
\[\norm{\partial_t n}_{L^{m}([0,T];L^{\infty}(\RR^d))}\leq \frac{C(T)m}{4-d}
\]
where $C(T)$ depends on $\norm{p}_{L^{\infty}(Q_T)}, \norm{\nabla p}_{L^4(Q_T)},$ and $\norm{n}_{L^{\infty}([0,T];W^{1,\infty}(\RR^d))}.$
\end{lemma}

\begin{proof}
For convenience we write $v=\partial_t n$ and note that $v$ solves the equation $\partial_t v-\Delta v=-\zeta$ where $\zeta=n\Delta p+\rho v +\rho n^2$.
Given a test function $\vp\in C^{\infty}_c(Q_T)$ and any time $t\geq 0$, the Duhamel formula gives us 
\[
\int_{Q_T} v(t,x)\vp(t,x)\, dx=\int_0^T\int_{\RR^d} v(0,x) e^{t\Delta} \vp(t,x)\, dx\, dt-\int_0^T\int_0^t\int_{\RR^d} \zeta(s,x) e^{(t-s)\Delta}\vp(t,x)\, ds\, dx \, dt.
\]

Using the expansions $n\Delta p=\Delta (pn)-2\nabla n\cdot \nabla p-p\Delta n$ and $\Delta n=v+\rho n$ we have 
\[
\zeta=\Delta (pn)-2\nabla n\cdot \nabla p+(\rho-p) v+\rho n(n-p).
\]
The last two terms in $\zeta$ are easy to estimate, so we ignore them and focus on $\Delta (pn)$ and $2\nabla n\cdot \nabla p$.  Using Holder's inequality and then Young's convolution inequality we see that
\[
|\int_0^T\int_0^t\int_{\RR^d} (\nabla p\cdot \nabla n)e^{(t-s)\Delta}\vp(t,x)\, ds\, dx \, dt|\leq \norm{\nabla n}_{L^{\infty}([0,T]\times\RR^d)}\norm{\nabla p}_{L^{4}([0,T]\times\RR^d)}\int_0^T \norm{e^{(t-s)\Delta}\vp}_{L^{4/3}([0,t]\times\RR^d)}
\]
\[
\lesssim \frac{1}{4-d}\norm{\nabla n}_{L^{\infty}([0,T]\times\RR^d)}\norm{\nabla p}_{L^{4}([0,T]\times\RR^d)}\norm{\vp}_{L^1([0,T]\times\RR^d)}.
\]
To estimate $\Delta (pn)$, we fix some $\alpha\leq 1-\frac{d}{4}$ and write
\[
|\int_0^T\int_0^t\int_{\RR^d} \Delta (np)e^{(t-s)\Delta}\vp(t,x)\, dx \, ds\,  dt|=|\int_0^T\int_0^t\int_{\RR^d} \Delta^{\alpha/2}(np)(\Delta^{1-\alpha/2}e^{(t-s)\Delta}\vp)\,  dx\, ds\, dt|.
\]
Up to constants, the previous line is bounded above by
\[
 \int_0^T\int_0^t \norm{n(s,\cdot)p(s,\cdot)}_{C^{0,\alpha}(\RR^d)}\norm{\Delta^{1-\alpha/2}e^{(t-s)\Delta}\vp(t,\cdot)}_{L^1(\RR^d)}\, ds\, dt
\]
We can then interpolate
\[
\norm{n p}_{C^{0,\alpha}(\{s\}\times\RR^d)}\lesssim \norm{n p}_{L^{\infty}(\{s\}\times\RR^d)}^{1-\frac{\alpha}{1-\frac{d}{4}}}\norm{n p}_{C^{0,1-\frac{d}{4}}(\{s\}\times\RR^d)}^{\frac{\alpha}{1-\frac{d}{4}}}\lesssim  
\]
\[
\norm{n p}_{L^{\infty}(\{s\}\times\RR^d)}^{1-\frac{\alpha}{1-\frac{d}{4}}}\big(\norm{n}_{L^{\infty}(\{s\}\times\RR^d)}\norm{\nabla p}_{L^4(\{s\}\times\RR^d)}+\norm{p}_{L^{\infty}(\{s\}\times\RR^d)}\norm{\nabla n}_{L^4(\{s\}\times\RR^d)} \big)^{\frac{\alpha}{1-\frac{d}{4}}}
\]

Therefore, by Young's convolution inequality
\[
 \int_0^T\int_0^t \norm{n(s,\cdot)p(s,\cdot)}_{C^{0,\alpha}(\RR^d)}\norm{\Delta^{1-\alpha/2}e^{(t-s)\Delta}\vp(t,\cdot)}_{L^1(\RR^d)}\, ds\, dt\lesssim 
 \]
 \[
 \norm{p}_{L^4([0,T];W^{1,4}(\RR^d))\cap L^{\infty}([0,T]\times\RR^d)}\norm{n}_{L^{\infty}([0,T];W^{1,\infty}(\RR^d))}\norm{\vp(t,\cdot)}_{L^{\frac{4-d}{4-d-4\alpha}}([0,t];L^1(\RR^d))}\int_0^T (t-s)^{1-\alpha/2}\, 
\]
Thus,
\[
|\int_0^T\int_0^t\int_{\RR^d} \Delta (np)e^{(t-s)\Delta}\vp(t,x)\, dx \, ds\,  dt|\lesssim \frac{1}{\alpha} \norm{p}_{L^4([0,T];W^{1,4}(\RR^d))\cap L^{\infty}([0,T]\times\RR^d)}\norm{n}_{L^{\infty}([0,T];W^{1,\infty}(\RR^d))}\norm{\vp(t,\cdot)}_{L^{\frac{4-d}{4-d-4\alpha}}([0,t];L^1(\RR^d))}
\]
The result now follows from choosing $\alpha$ such that $\frac{m}{m-1}=1+\frac{\alpha}{4-d-4\alpha}$ and taking the supremum over $\vp$ in the unit ball of $L^{1+\frac{\alpha}{4-d-\alpha}}([0,T];L^1(\RR^d))$.
\end{proof}

\textcolor{blue}{Remark: This is probably not the optimal way to estimate $\nabla \log(n), \partial_t \log(n), \Delta \log(n)$, probably better to analyze the equation satisfied by $\log(n)$, but the equation is nonlinear and doesn't have a simple Duhamel formula.}




We now combine Lemmas \ref{lem:ab}, \ref{lem:dt_n_estimate} and \ref{lem:nutrient_lower_bound} to establish super exponential control (in space) on $u_+$.

\textcolor{blue}{can you explain more why (2.7) is the optimal growth estimate one can get from previous lemmas?}

\begin{prop}
    Under our previous assumptions, for any $T>0$ there exists a constant $b>0$ and $C(T)>0$ such that
    \begin{equation}
        \int_0^T \exp\Big(\log\big(\norm{\exp( b u_+^2)}_{L^1(\{t\}\times\RR^d)}\big)^{1/2}\Big)\, dt\leq C(T).
    \end{equation}
\end{prop}
\begin{proof}
    From Lemma \ref{lem:ab} and the fact that $G=n$, we have the control
 \[
   \frac{d}{dt}\int_{\RR^d}\gi  f(u)+\int_{\RR^d} f^*(f'(u))(\gi u+\frac{n}{2})+4 f'(u)|D^2p|^2+p f''(u)|\nabla u|^2\leq 
   \]
   \[
  \int_{\RR^d} \frac{4}{\gamma}f(u)(\gi u+n)+4pf''(u)|\nabla G|^2+\frac{n}{2}f(\frac{4p\Delta n+2\partial_t n}{n})
\]
 for any convex function $f$.  Integrating both sides with respect to time we get 
  \[
   \frac{d}{dt}\int_{\RR^d}\gi  f(u)+\int_{\RR^d} f^*(f'(u))(\gi u+\frac{n}{2})+4 f'(u)|D^2p|^2+p f''(u)|\nabla u|^2\leq 
   \]
   \[
  \int_{\RR^d} \frac{4}{\gamma}f(u)(\gi u+n)+4pf''(u)|\nabla G|^2+\frac{n}{2}f(\frac{4p\Delta n+2\partial_t n}{n})
\]
  Fix some $b>0$ and choose $f(a)=\exp(ba_+^2)-1$.  Note that for $a\geq 0$, $f''(a)=4b^2a^2\exp(ba^2)+2b\exp(ba^2)$ and $f^*(f'(a))=2ba^2\exp(ba^2)-\exp(ba^2)+1$.  If we choose $b$ such that $\frac{\bar{n}(t)}{2}-2b\norm{p|\nabla G|^2}_{L^{\infty}([0,T]\times\RR^d)}>0$, then $f^*(f'(u))(\gi u+\frac{n}{2})$ dominates $4pf''(u)|\nabla G|^2$ and we obtain superexponential control on $u_+$ provided that we can control $\frac{n}{2}f(\frac{4p\Delta n+2\partial_t n}{n})$, however this follows from our bound on $\norm{\partial_t n}_{L^{\infty}(\RR^d)}$
\end{proof}




\begin{prop}
If $d<4$ and $(\rho, p,n)$ is a weak solution to the system
\[
\partial_t \rho-\nabla \cdot (\rho \nabla p)=\rho n, \quad \rho\leq 1, \; p(1-\rho)=0,
\]
\[
\partial_t n-\Delta n=-\rho n,
\]
with initial data $n_0\in W^{1,\infty}(\RR^d)$ and $\rho_0\in L^1(\RR^d;\{0,1\})$, then
$p$ weakly satisfies the differential inequality
\[
\partial_t p-|\nabla p|^2\geq \lambda p
\]
where $\lambda$ is a nonnegative function of time such that $\lambda\in L^m([0,T])$ for any $m\in [1,\infty)$ and $T\geq 0$.
\end{prop}
\begin{proof}
For each $j\in \ZZ_+$ define $\rho_{0,j}=K_{1/j}*\rho_0$ and $n_{j}=K_{1/j}*n$ where $K$ is the heat kernel of width $1/j$.
Next, let $(\rho_{j}, p_{j})$ be a weak solution to the equation
\[
\partial_t \rho_{j}-\nabla \cdot (\rho_{j}\nabla p_{j})=\rho_{j}n_{j} \quad p_{j}=\rho_{j}^{j}
\]
Since $n_j$ is smooth and $\rho_j$ is bounded away from zero on any compact set $E\subset Q_{\infty}$ it follows that $(\rho_j, p_j)\in C^{\infty}(E)$.  Hence, $p_j$ is a smooth solution to the equation
\[
\partial_t p_j-|\nabla p_j|^2-jp_j(\Delta p_j+n_j)=0
\]

Set $u_j=-j(\Delta p_j+n_j)$.  Let $f_k:\RR\to\RR$ be the function $f_k(a)=\frac{1}{k+1}\max(a,0)^{k+1}$.  By Lemma \ref{lem:ab}, we have 
\begin{multline}\label{eq:u_nutrient_estimate}
   \frac{d}{dt}\int_{\RR^d}\frac{1}{j(k+1)}  (u_j)_+^{k+1}+\int_{\RR^d} \frac{k-2/j}{k+1}(u_j)_+^{k+1}(\frac{1}{j} (u_j)_++n_j)+2 (u_j)_+^k|D^2p_j|^2+\frac{k}{2}p (u_j)_+^{k-1}|\nabla u_j|^2\\
 \leq \int_{\RR^d}2kp_j(u_j)_+^{k-1}|\nabla n_j|^2-(u_j)_+^k(2p_j\Delta n_j+\partial_t n_j).
\end{multline}
After integrating in time, dropping favorable terms, and assuming that $k, j\geq 3$, we see that 
\begin{multline}\label{eq:u_nutrient_estimate}
  \int_{Q_T} \frac{n_j}{2}(u_j)_+^{k+1}
 \leq \frac{1}{j(k+1)}\norm{(u_j)_+}_{\{0\}\times\RR^d}^{k+1} + \int_{Q_T}2kp_j(u_j)_+^{k-1}|\nabla n_j|^2-(u_j)_+^k(2p_j\Delta n_j+\partial_t n_j).
\end{multline}
Using Lemma \ref{lem:dt_n_estimate}, it follows that 
\[
c_j(T)\norm{(u_j)_+}_{L^{k+1}(\RR^d)}^{2}+\lesssim 2k+\norm{(u_j)_+}_{L^k(\RR^d)}\norm{\partial_t n}_{L^{\infty}(\RR^d)}
\]
\end{proof}

